Cache-Enabled Broadcast Packet Erasure Channels with State Feedback

We consider a cache-enabled K-user broadcast erasure packet channel in which a server with a library of N files wishes to deliver a requested file to each user who is equipped with a cache of a finite memory M. Assuming that the transmitter has state feedback and user caches can be filled during off-peak hours reliably by decentralized cache placement, we characterize the optimal rate region as a function of the memory size, the erasure probability. The proposed delivery scheme, based on the scheme proposed by Gatzianas et al., exploits the receiver side information established during the placement phase. Our results enable us to quantify the net benefits of decentralized coded caching in the presence of erasure. The role of state feedback is found useful especially when the erasure probability is large and/or the normalized memory size is small.

==> macros.tex <==
%\pagestyle{myheadings}

%
\newcommand{\RED}{\color[rgb]{0.69,0,0}}
\newcommand{\BLUE}{\color[rgb]{0,0,0.69}}
\newcommand{\GREEN}{\color[rgb]{0,0.69,0}}

\setlength\unitlength{1mm}

%
%\newcommand{\insertfig}[3]{
%\begin{figure}[tbp]\begin{center}\begin{picture}(120,90)
%\put(0,-5){\includegraphics[width=12cm,height=9cm,clip=]{#1.eps}}\end{picture}\end{center}
%\caption{#2}\label{#3}\end{figure}}

%
%\newcommand{\inserttwofig}[4]{
%\begin{figure}\begin{center}\begin{picture}(150,170)
%\put(10,80){\includegraphics[with=8.5cm]{#1.ps}}
%\put(10, 0){\includegraphics[with=8.5cm]{#2.ps}}
%\end{picture}\end{center}
%\caption{#3}\label{#4}\end{figure}}

% bb font symbols

\newfont{\bbb}{msbm10 scaled 500}
\newcommand{\CCC}{\mbox{\bbb C}}


\newfont{\bb}{msbm10 scaled 1100}
\newcommand{\CC}{\mbox{\bb C}}
\newcommand{\RR}{\mbox{\bb R}}
\newcommand{\ZZ}{\mbox{\bb Z}}
\newcommand{\FF}{\mbox{\bb F}}
\newcommand{\GG}{\mbox{\bb G}}

\newcommand{\Pout}{P_{\rm out}}
\newcommand{\PP}{\mathbb{P}}
% Vectors

\newcommand{\av}{{\bf a}}
\newcommand{\bv}{{\bf b}}
\newcommand{\cv}{{\bf c}}
\newcommand{\dv}{{\bf d}}
\newcommand{\ev}{{\bf e}}
\newcommand{\fv}{{\bf f}}
\newcommand{\gv}{{\bf g}}
\newcommand{\hv}{{\bf h}}
\newcommand{\iv}{{\bf i}}
\newcommand{\jv}{{\bf j}}
\newcommand{\kv}{{\bf k}}
\newcommand{\lv}{{\bf l}}
\newcommand{\mv}{{\bf m}}
\newcommand{\nv}{{\bf n}}
\newcommand{\ov}{{\bf o}}
\newcommand{\pv}{{\bf p}}
\newcommand{\qv}{{\bf q}}
\newcommand{\rv}{{\bf r}}
\newcommand{\sv}{{\bf s}}
\newcommand{\tv}{{\bf t}}
\newcommand{\uv}{{\bf u}}
\newcommand{\wv}{{\bf w}}
\newcommand{\vv}{{\bf v}}
\newcommand{\xv}{{\bf x}}
\newcommand{\yv}{{\bf y}}
\newcommand{\zv}{{\bf z}}
\newcommand{\zerov}{{\bf 0}}
\newcommand{\onev}{{\bf 1}}

% Matrices

\newcommand{\Am}{{\bf A}}
\newcommand{\Bm}{{\bf B}}
\newcommand{\Cm}{{\bf C}}
\newcommand{\Dm}{{\bf D}}
\newcommand{\Em}{{\bf E}}
\newcommand{\Fm}{{\bf F}}
\newcommand{\Gm}{{\bf G}}
\newcommand{\Hm}{{\bf H}}
\newcommand{\Id}{{\bf I}}
\newcommand{\Jm}{{\bf J}}
\newcommand{\Km}{{\bf K}}
\newcommand{\Lm}{{\bf L}}
\newcommand{\Mm}{{\bf M}}
\newcommand{\Nm}{{\bf N}}
\newcommand{\Om}{{\bf O}}
\newcommand{\Pm}{{\bf P}}
\newcommand{\Qm}{{\bf Q}}
\newcommand{\Rm}{{\bf R}}
\newcommand{\Sm}{{\bf S}}
\newcommand{\Tm}{{\bf T}}
\newcommand{\Um}{{\bf U}}
\newcommand{\Wm}{{\bf W}}
\newcommand{\Vm}{{\bf V}}
\newcommand{\Xm}{{\bf X}}
\newcommand{\Ym}{{\bf Y}}
\newcommand{\Zm}{{\bf Z}}

% Calligraphic

\newcommand{\Ac}{{\cal A}}
\newcommand{\Bc}{{\cal B}}
\newcommand{\Cc}{{\cal C}}
\newcommand{\Dc}{{\cal D}}
\newcommand{\Ec}{{\cal E}}
\newcommand{\Fc}{{\cal F}}
\newcommand{\Gc}{{\cal G}}
\newcommand{\Hc}{{\cal H}}
\newcommand{\Ic}{{\cal I}}
\newcommand{\Jc}{{\cal J}}
\newcommand{\Kc}{{\cal K}}
\newcommand{\Lc}{{\cal L}}
\newcommand{\Mc}{{\cal M}}
\newcommand{\Nc}{{\cal N}}
\newcommand{\Oc}{{\cal O}}
\newcommand{\Pc}{{\cal P}}
\newcommand{\Qc}{{\cal Q}}
\newcommand{\Rc}{{\cal R}}
\newcommand{\Sc}{{\cal S}}
\newcommand{\Tc}{{\cal T}}
\newcommand{\Uc}{{\cal U}}
\newcommand{\Wc}{{\cal W}}
\newcommand{\Vc}{{\cal V}}
\newcommand{\Xc}{{\cal X}}
\newcommand{\Yc}{{\cal Y}}
\newcommand{\Zc}{{\cal Z}}
\newcommand{\HHc}{{\bf \Hc}}
% Bold greek letters

\newcommand{\alphav}{\hbox{\boldmath$\alpha$}}
\newcommand{\betav}{\hbox{\boldmath$\beta$}}
\newcommand{\gammav}{\hbox{\boldmath$\gamma$}}
\newcommand{\deltav}{\hbox{\boldmath$\delta$}}
\newcommand{\etav}{\hbox{\boldmath$\eta$}}
\newcommand{\lambdav}{\hbox{\boldmath$\lambda$}}
\newcommand{\epsilonv}{\hbox{\boldmath$\epsilon$}}
\newcommand{\nuv}{\hbox{\boldmath$\nu$}}
\newcommand{\muv}{\hbox{\boldmath$\mu$}}
\newcommand{\zetav}{\hbox{\boldmath$\zeta$}}
\newcommand{\phiv}{\hbox{\boldmath$\phi$}}
\newcommand{\psiv}{\hbox{\boldmath$\psi$}}
\newcommand{\thetav}{\hbox{\boldmath$\theta$}}
\newcommand{\tauv}{\hbox{\boldmath$\tau$}}
\newcommand{\omegav}{\hbox{\boldmath$\omega$}}
\newcommand{\xiv}{\hbox{\boldmath$\xi$}}
\newcommand{\sigmav}{\hbox{\boldmath$\sigma$}}
\newcommand{\piv}{\hbox{\boldmath$\pi$}}
\newcommand{\Gammam}{\hbox{\boldmath$\Gamma$}}
\newcommand{\Lambdam}{\hbox{\boldmath$\Lambda$}}
\newcommand{\Deltam}{\hbox{\boldmath$\Delta$}}
\newcommand{\Sigmam}{\hbox{\boldmath$\Sigma$}}
\newcommand{\Phim}{\hbox{\boldmath$\Phi$}}
\newcommand{\Pim}{\hbox{\boldmath$\Pi$}}
\newcommand{\Psim}{\hbox{\boldmath$\Psi$}}
\newcommand{\Thetam}{\hbox{\boldmath$\Theta$}}
\newcommand{\Omegam}{\hbox{\boldmath$\Omega$}}
\newcommand{\Xim}{\hbox{\boldmath$\Xi$}}

\newcommand{\Eta}{\hbox{$\eta$}}
% mixed symbols

\newcommand{\sinc}{{\hbox{sinc}}}
\newcommand{\diag}{{\hbox{diag}}}
\renewcommand{\det}{{\hbox{det}}}
\newcommand{\trace}{{\hbox{tr}}}
\newcommand{\rank}{{\hbox{rank}}}
\newcommand{\cov}{{\hbox{cov}}}
\newcommand{\sign}{{\hbox{sign}}}
\renewcommand{\arg}{{\hbox{arg}}}
\newcommand{\var}{{\hbox{var}}}
\newcommand{\SINR}{\hbox{SINR}}
\newcommand{\SNR}{\hbox{SNR}}
\newcommand{\EE}{\hbox{E}}
\newcommand{\Ei}{{\rm E}_{\rm i}}
\renewcommand{\Re}{{\rm Re}}
\renewcommand{\Im}{{\rm Im}}
\newcommand{\eqdef}{\stackrel{\Delta}{=}}
\newcommand{\<}{\left\langle}
\renewcommand{\>}{\right\rangle}

% More symbols

\newcommand{\Ph}{\widehat{P}}
\newcommand{\tauvh}{\widehat{\tauv}}
\newcommand{\tauh}{\widehat{\tau}}
\newcommand{\ct}{\widetilde{c}}
\newcommand{\xt}{\widetilde{x}}
\newcommand{\zt}{\widetilde{z}}
\newcommand{\st}{\widetilde{s}}
\newcommand{\ch}{\widehat{c}}
\newcommand{\bh}{\widehat{b}}
\newcommand{\cvt}{\widetilde{\cv}}
\newcommand{\cvh}{\widehat{\cv}}
\newcommand{\dvh}{\widehat{\dv}}
\newcommand{\bvh}{\widehat{\bv}}
\newcommand{\xvh}{\widehat{\xv}}
\newcommand{\svh}{\widehat{\sv}}
\newcommand{\jh}{\widehat{j}}
\newcommand{\gh}{\widehat{g}}
\newcommand{\gvh}{\widehat{\gv}}
\newcommand{\gvhh}{\widehat{\gvh}}
\newcommand{\hvh}{\widehat{\hv}}
\newcommand{\xh}{\widehat{x}}
\newcommand{\zvo}{\overline{\zv}}
\newcommand{\ao}{\overline{a}}
\newcommand{\bo}{\overline{b}}
\newcommand{\zo}{\overline{z}}
\newcommand{\xo}{\overline{x}}
\newcommand{\vo}{\overline{v}}
\newcommand{\vvo}{\overline{\vv}}
\newcommand{\gvo}{\overline{\gv}}
\newcommand{\hvo}{\overline{\hv}}
\newcommand{\cvo}{\overline{\cv}}
\newcommand{\yvt}{\widetilde{\yv}}
\newcommand{\svt}{\widetilde{\sv}}
\newcommand{\nuvt}{\widetilde{\nuv}}
\newcommand{\dvt}{\widetilde{\dv}}
\newcommand{\Rmt}{\widetilde{\Rm}}
\newcommand{\Rmh}{\widehat{\Rm}}
\newcommand{\Dmt}{\widetilde{\Dm}}
\newcommand{\Kt}{\widetilde{K}}
\newcommand{\Lt}{\widetilde{L}}
%\newcommand{\Pt}{\widetilde{P}}
\newcommand{\yt}{\widetilde{y}}
\newcommand{\bt}{\widetilde{b}}
\newcommand{\et}{\widetilde{e}}
\newcommand{\Jt}{\widetilde{J}}
\newcommand{\Et}{\et_0}
\newcommand{\hvt}{\widetilde{\hv}}

